Enhancing Scalability and Performance in Influence Maximization with Optimized Parallel Processing

Influence Maximization (IM) is vital in viral marketing and biological network analysis for identifying key influencers. Given its NP-hard nature, approximate solutions are employed. This paper addresses scalability challenges in scale-out shared memory system by focusing on the state-of-the-art Influence Maximization via Martingales (IMM) benchmark. To enhance the work efficiency of the current IMM implementation, we propose EFFICIENTIMM with key strategies, including new parallelization scheme, NUMA-aware memory usage, dynamic load balancing and fine-grained adaptive data structures. Benchmarking on a 128-core CPU system with 8 NUMA nodes, EFFICIENTIMM demonstrated significant performance improvements, achieving an average 5.9x speedup over Ripples across 8 diverse SNAP datasets, when compared to the best execution times of the original Ripples framework. Additionally, on the Youtube graph, EFFICIENTIMM demonstrates a better memory access pattern with 357.4x reduction in L1+L2 cache misses as compared to Ripples.

==> discussion.tex <==
\section{Discussion and Future Work}
\ju{We can reduce and merge this section to Related work section.}
This section describes our investigation into potential performance benefits and identifies critical bottlenecks within the IMM framework. 
As highlighted in previous section~\ref{sec:motivation}, \textit{Find\_Most\_Influential\_Set} was initially the primary bottleneck, hindering IMM's scalability. 
\sys enhances IMM by increasinrg the scalability of \textit{Find\_Most\_Influential\_Set}, which now performs 5.9 times faster than Ripples on average. 
As a result, \textit{Generate\_RRRSet} has emerged as the new bottleneck in IMM. 
We propose several potential directions for further performance improvements:

% \noindent
% \textbf{NUMA-Awareness: }
% Our profiling shows that over 60\% of the performance overhead in \textit{Generate\_RRR\_Set} occurs when checking the bitmap that stores visited vertices in BFS (line 8 of Algorithm~\ref{alg:bfs_diffusion}). 
% To alleviate this issue, we located the bitmap closer to the processor, ensuring that each NUMA node operates within its local memory as much as possible. 
% By leveraging \textit{mbind}, we achieved a minor performance increase. However, this adjustment did not fully resolve the bottleneck as checking the neighbors of certain vertices has become the new constraint. 
% A better graph storage method that considers NUMA effects is essential for further improvements.

\noindent
\textbf{Effective BFS: }
To further accelerate BFS, we are exploring two potential approaches: 
Firstly, community-based sorting, which organizes nodes by community to preserve locality and minimize cache misses, enhancing computational efficiency. Secondly, Multi-Source BFS initiates traversal from multiple sources, merging traversal fronts when they converge at the same vertex. This merging reduces redundant computations and improves efficiency by preventing duplicated vertex access~\cite{neff2023fused}.

\noindent
\textbf{Online Sampling: }
Reducing the workload through more efficient sampling techniques has realistic meaning with the specific user applications.
OPIM leveraged the IMM workflow and introduced an online algorithm that permits users to halt the sampling process prematurely if the initial sampling exceeds their requirements \cite{tang2018OPIM}. Addressing the challenges posed by extensive sampling in the standard IMM algorithm, OPIM offers enhanced flexibility, allowing for adaptation to diverse contexts. Maintaining the IMM workflow, our proposed \sys is designed for smooth adaptation to the OPIM model, which extends its use cases.

While the main focus of \sys is orthogonal to these optimizations, integrating these enhancements could potentially boost the overall performance of IMM. 
Each proposed solution aims to tackle the specific challenges identified in our profiling, paving the way for a more robust and scalable implementation.
